Hierarchical Federated Learning through LAN-WAN Orchestration

Federated learning (FL) was designed to enable mobile phones to collaboratively learn a global model without uploading their private data to a cloud server. However, exiting FL protocols has a critical communication bottleneck in a federated network coupled with privacy concerns, usually powered by a wide-area network (WAN). Such a WAN-driven FL design leads to significantly high cost and much slower model convergence. In this work, we propose an efficient FL protocol, which involves a hierarchical aggregation mechanism in the local-area network (LAN) due to its abundant bandwidth and almost negligible monetary cost than WAN. Our proposed FL can accelerate the learning process and reduce the monetary cost with frequent local aggregation in the same LAN and infrequent global aggregation on a cloud across WAN. We further design a concrete FL platform, namely LanFL, that incorporates several key techniques to handle those challenges introduced by LAN: cloud-device aggregation architecture, intra-LAN peer-to-peer (p2p) topology generation, inter-LAN bandwidth capacity heterogeneity. We evaluate LanFL on 2 typical Non-IID datasets, which reveals that LanFL can significantly accelerate FL training (1.5x-6.0x), save WAN traffic (18.3x-75.6x), and reduce monetary cost (3.8x-27.2x) while preserving the model accuracy.

==> eval-acc-time-lan-num.tex <==
% !TeX root = main.tex

\begin{figure}[t]
	\centering
	\begin{minipage}[b]{0.24\textwidth}
	\includegraphics[width=1.0\textwidth]{figs/eval-acc-time-lan-num-celeba}
	%\vspace*{-.6cm}
	\subcaption{Celeba}
	\end{minipage}
    ~
	\begin{minipage}[b]{0.24\textwidth}
	\includegraphics[width=1.0\textwidth]{figs/eval-acc-time-lan-num-femnist}
	%\vspace*{-.6cm}
	\subcaption{FEMNIST}
	\end{minipage}
	\caption{acc-time-num. LAN-FL setting: E=2,RL=5,BL=20. LEAF setting: E=10,BW=2}
	\label{fig:eval-acc-time-lan-num}
\end{figure}


==> eval-throughput-devices.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=0.4\textwidth]{figs/eval-throughput-devices}
	%\vspace*{-.6cm}
	\label{fig:eval-throughput-devices}
    \caption{throughput-devices}
\end{figure} 

==> eval-time-device-band-celeba.tex <==
% !TeX root = main.tex

\begin{figure}[t]
	\centering
    \begin{minipage}[b]{0.24\textwidth}
	\includegraphics[width=1.0\textwidth]{figs/eval-time-num-celeba}
	%\vspace*{-.6cm}
	\subcaption{lan-num-celeba}
	\end{minipage}
    ~
    \begin{minipage}[b]{0.24\textwidth}
	\includegraphics[width=1.0\textwidth]{figs/eval-time-num-femnist}
	%\vspace*{-.6cm}
	\subcaption{lan-num-femnist}
	\end{minipage}
    \caption{time-num-lan}
    \label{fig:eval-time-num-lan}
\end{figure} 

==> eval-traffic.tex <==
% !TeX root = main.tex

\begin{figure}[t]
	\centering
	\includegraphics[width=0.4\textwidth]{figs/eval-traffic}
	%\vspace*{-.6cm}
    \caption{Traffic}
	\label{fig:eval-traffic}
\end{figure} 


==> evidence.tex <==

\mwx{The new evidence below. Note: they are not wireless; it's affected by coronavirus.}

\paragraph{A campus case of cold videos}
As supporting evidence, we collected video query data from a campus the authors affiliated with.
Occupying around 2 km$^2$ area, the campus is equipped with more than 1,800 (950) outdoor (indoor) surveillance cameras.
Currently, all captured videos are streamed to an edge server, stored for 2--3 months, and queried retrospectively.
The queries are mostly ML-based, e.g., object detection or license plate recognition, but also support manual inspection.
During the 2-months data collection period, only 3 queries are executed that span 0.65\% cameras and 0.0018\% video data generated.
Based on the collected data, we estimate that more than 99.9\% videos remain cold and will never be queried.


==> fig-traffic.tex <==
% !TeX root = main.tex

\begin{figure}[t]
	\centering
	\includegraphics[width=1.0\textwidth]{figs/eval-traffic}
	\caption{The on-client cost reduction brought by our key optimizations (``DRN'': dynamic round number; ``ERC'': early dropping candidates; ``Group'': parallel training).
		The setting is the same as Figure. The y-axis is logarithmic.}
	\label{fig:traffic}
\end{figure}

==> tab-result-traffic.tex <==
% !TeX root = main.tex

\begin{table}[t]
\footnotesize
\begin{tabular}{|c|L{2.9cm}|L{1.4cm}|L{1.4cm}|}
	\hline
	\multicolumn{1}{|l|}{\textbf{Dataset}} & \textbf{FL} & \textbf{Accuracy (\%)} & \textbf{Traffic(MB)} \\ \hline \hline
	
	\multirow{4}{*}{FEMNIST} & \textbf{LEAF(E=1)} & \textbf{68.8 (0.0)} & \textbf{70.3 (0.0)} \\ \cline{2-4}
	& \textbf{LEAF(E=10)} & \textbf{68.8 (0.0)} & \textbf{70.3 (0.0)} \\ \cline{2-4}
	& LAN-FL(E=2 RL=5) & 68.5 & 9.8 \\ \hline \hline

    \multirow{4}{*}{CelebA} & \textbf{LEAF(E=1)} & \textbf{68.8 (0.0)} & \textbf{70.3 (0.0)} \\ \cline{2-4}
	& \textbf{LEAF(E=20)} &  \textbf{68.8 (0.0)} & \textbf{70.3 (0.0)} \\ \cline{2-4}
	& LAN-FL(E=2 RL=10) & 68.5 & 9.8 \\ \hline \hline
	
\end{tabular}
\caption{traffic}
\label{tab:result-traffic}
\end{table}

==> terms.tex <==
% !TeX root = main.tex

% -------------------TERMS -------------------

\newcommand{\secenv}{secure environment}
\newcommand{\unsecenv}{normal environment}

\newcommand{\se}{secure world}
\newcommand{\te}{secure world}
\newcommand{\Te}{Secure world}
\newcommand{\Se}{Secure world}
\newcommand{\nw}{normal world}
\newcommand{\sw}{secure world}


\newcommand{\cc}{cascading container}
\newcommand{\ccs}{cascading containers}
\newcommand{\Cc}{Cascading container}


%\newcommand{\subuf}{sequential batch}
%\newcommand{\ubuf}{batch}
%\newcommand{\Ubuf}{Batches}

\newcommand{\subuf}{unbounded array}
\newcommand{\ubuf}{uArray}
\newcommand{\Ubuf}{Batches}

\newcommand{\tee}{trusted execution environment}

\newcommand{\down}{\textit{down}}

\newcommand{\wm}{watermark}
\newcommand{\Wm}{Watermark}

\newcommand{\multicore}{multicore}

% --- machines --- 
%\newcommand{\makalu}{R930}
%\newcommand{\ktwo}{R720}
\newcommand{\makalu}{56CM}
\newcommand{\ktwo}{12CM}

% --- design terms --- 

% --- benchmarks --- 
\newcommand{\jacksonh}{JacksonH}
\newcommand{\jacksont}{JacksonT}
\newcommand{\banff}{Banff}
\newcommand{\mierlo}{Mierlo}
\newcommand{\miami}{Miami}
\newcommand{\ashland}{Ashland}
\newcommand{\shibuya}{Shibuya}

\newcommand{\chaweng}{Chaweng}
\newcommand{\lausanne}{Lausanne}
\newcommand{\venice}{Venice}
\newcommand{\tucson}{Tucson}
\newcommand{\oxford}{Oxford}
\newcommand{\whitebay}{Whitebay}


\newcommand{\coralreef}{CoralReef}
\newcommand{\boathouse}{BoatHouse}

\newcommand{\eagle}{Eagle}



%\newcommand{\filter}{\code{filter}}
%\newcommand{\winsum}{\code{winsum}}
%\newcommand{\join}{\code{join}}
%\newcommand{\unique}{\code{unique}}
%\newcommand{\freq}{\code{freq}}
%\newcommand{\grid}{\code{grid}}

\newcommand{\frontend}{camera execution}
\newcommand{\backend}{cloud execution}

\newcommand{\countmax}{max Count}
\newcommand{\countavgmedian}{average/median Count}


%\newcommand{\OpF}{Op\textsubscript{F}}
%\newcommand{\OpS}{Op\textsubscript{S}}

%\newcommand{\OpF}{O\textsubscript{FAST}}
%\newcommand{\OpS}{O\textsubscript{SLOW}}

%\newcommand{\OpF}{O\textsubscript{CHEAP}}
%\newcommand{\OpS}{O\textsubscript{EXP}}

\newcommand{\OpF}{E\textsubscript{CHEAP}}
\newcommand{\OpS}{E\textsubscript{EXP}}

\newcommand{\OpFprime}{E\textsubscript{CHEAP}'}
\newcommand{\OpSprime}{E\textsuperscript{EXP}'}

% --- exp --- 
\newcommand{\cloudonly}{\code{CloudOnly}}
\newcommand{\noscope}{\code{OptOp}}
\newcommand{\focus}{\code{PreIndexAll}}

\newcommand{\extlat}{externalization latency}
%% ----------------------------------------------
